DRAGNN: A Transition-based Framework for Dynamically Connected Neural Networks

In this work, we present a compact, modular framework for constructing novel recurrent neural architectures. Our basic module is a new generic unit, the Transition Based Recurrent Unit (TBRU). In addition to hidden layer activations, TBRUs have discrete state dynamics that allow network connections to be built dynamically as a function of intermediate activations. By connecting multiple TBRUs, we can extend and combine commonly used architectures such as sequence-to-sequence, attention mechanisms, and re-cursive tree-structured models. A TBRU can also serve as both an encoder for downstream tasks and as a decoder for its own task simultaneously, resulting in more accurate multi-task learning. We call our approach Dynamic Recurrent Acyclic Graphical Neural Networks, or DRAGNN. We show that DRAGNN is significantly more accurate and efficient than seq2seq with attention for syntactic dependency parsing and yields more accurate multi-task learning for extractive summarization tasks.

==> tex/backup.tex <==
% this section contains a dump of old text that might be useful again.

The interesting property of TBRU's is thatd
It's easy to see that There's several important properties of TBRUs that distinguish them from other recurrent network frameworks. 

input function $\bm$, and a RNN cell $\mathbf{RNN}$, a

The typical story for recurrent neural networks is as follows
[following notation in Wiseman \& Rush 2016]. Let $\bm_1, \dots, \bm_n$ be a
series of input vectors, and $\bh_0$ a pre-specified initial hidden state
vector. A recurrent neural network recursively computes hidden states at each
time step:
\begin{equation}
  \bh_i \leftarrow \mathbf{RNN}(\bm_i, \bh_{i-1}; \theta).
\end{equation}
If we use the hidden states to predict labels The network is trained via some loss function over the hidden states, such as Learning recurrent networks Recurrent networks are typically used 


To apply recurrent models to transition systems, we will extend this definition
in two major ways:


we can assume that for every state in a decision sequence $s_i$ we have a
corresponding input vector $\bm(s_i)$. For example, $\bm(s_i)$ could be the
embedding vector of the $i$'th word in an input sequence (e.g. during encoding)
or the $i$'th symbol in an output sequence (e.g. during decoding). \lpk{for
  general transition system, the input might not be always at the $i$'th word
  when we at the $i$'th transition. So back to the point I think TBRU should be
  before the discussion of seq2seq?} Then we can define a recurrent scoring
function:
\begin{equation}
  \score(s_i, d;\bh_{i-1},\theta) = \bw_d^\top\mathbf{RNN}(\bm(s_i),\bh_{i-1};\theta),
\end{equation}
where we simply score decisions based on the corresponding hidden state. 

In this recurrent neural network model, inference can be summarized as follows:


To implement the classic seq2seq framework, we can implement two transition
systems: one for encoding and one for decoding. The encoder transition system is
simple:
\begin{itemize}
\item $s_i$ is just the input pointer $\{i\}$, which points to the next token to
  encode.
\item There is only one possible decision at each step, to advance the input
  pointer, i.e. $t(s_i,\cdot) = \{i+1\}$.
\item $\bm(s_i)$ is then just the embedding $\bm_i$ of the $i$'th input symbol.
\end{itemize}
 The decoder transition system, in turn, keeps track of the generated output sequence:
\begin{itemize}
\item $s_i$ contains emitted labels so far, i.e. $s_i = \{y_1, \dots, y_{i-1}\}$.
\item Each decision $d_i$ adds one additional generated token, i.e. $t(s_i,d) = \{y_1,\dots,y_{i-1},d\}$. 
\item The initial hidden state in the decoder $\bh_0$ is set to be some function
  of the final hidden layer $\bh^E_n$ of the encoding system.
\item The input $\bm(s_i)$ is the embedding $\bm_{y_{i-1}}$ of the output token at the
  previous position.
\end{itemize}

To summarize, in this transition-based implementation of seq2seq, there is an explicit devision of labor:
\begin{itemize}
\item The transition system manages the {\em discrete} state of each
  component. This discrete state is used to determine the input embedding $\bm$
  to the RNN and contains the discrete labels produced as output.
\item The RNN computes a {\em continuous} representation for each state, which
  is used as a representation of the input (via the encoder) and to predict the
  output (via the decoder).
\end{itemize}

We observe that both the encoder and decoder component of this transtion-based
seq2seq produces both continuous and discrete outputs: the representations from
the RNN cell and the discrete structure in the terminal transition state. We
call this functional unit, 

In the next section, we'll show how we can how we can define TBRU's
systematically to incorporate arbitrary structures on both inputs and
outputs. Furthermore, we will use this framework to generalize the notion of an
encoder/decoder framework to an arbitrary, dynamically computed graph of
representations that can be used to learn a single deep model for arbitrary sets
of NLP tasks.

\subsection{Dynamic recurrent acyclic graphical neural networks}

The transition systems described above are quite simple: we encode both the
input and the output as a sequence with no internal structure. However, for many
problems, it's known ahead of time that there is structure over the input,
output, or both. For example, models like SPINN [cite] or TreeLSTM [cite]
explicitly represent compositional inputs by utilizing predicted tree structures
in the input. [Give more examples of RNN's over structured inputs.] Meanwhile,
parsing models [Andor et al] use neural networks over transition systems to
produce tree structures as output. \lpk{The word ``structure'' here is a little unclear? In
TreeLSTM, the computation graph is actually recursive (the computation graph is constructed
based on the structure of the Tree). But in the DRAGNN framework, since we are doing transition
based systems. The structure of the computation graph is always sequential recurrent --
we are using TBRU.}

Our goal in this work is to show how we can re-use any transition system that
produces structured output to encode a (possibly compositional) continuous
representation of the input. As it turns out, we only need a few generalizations
beyond the basic TBRU described above.

The core idea is that we will move away from the explicit notion of an encoder
and a decoder. Instead, we use a set of TBRU-based components that encode both
continuous representations and discrete structure that are utilized as
needed. In the classic seq2seq model, we use the continuous representations of
the ``encoder'' TBRU to obtain the discrete structure from the ``decoder''
TBRU. Here, we allow arbitrary re-use of continuous or discrete structure of any
TBRU as long as the resulting computation forms a directed acyclic graph (DAG).

As we will see, this framework lets us use TBRU's to obtain models of arbitrary
compositionality and over arbitrary output structure. Furthermore, the basic
cell can be implemented efficiently in a generic fashion in almost any neural
network toolbox. The key is to obtaining such generic compositionality is to
allow both the recurrent structure and the input embeddings to be determined via
pre-specified functions of the discrete state.

Formally, we introduce the following:
\begin{itemize}
\item Assume an ordered set of $T$ TBRU components, which we will notate with
  superscript $1,\dots,T$, and so forth. We will execute each component in
  sequence, one at a time.
\item We define a global graph state $\GG_0 = \{\}$, and a global step
  $\alpha$. At each timestep $i$ of a given component $j$, we update the global
  state to store the hidden state from that component:
$$\GG_{\alpha+1} \leftarrow \GG_\alpha \cup \{\bh_i^j\}, \quad \alpha \leftarrow \alpha + 1$$
\item We update our definition of the RNN cell to include a function for
  determining the hidden layer representation. This new function $\br$ pulls a
  set of representations from the global state $\GG$ for a given time step
  $\alpha$ (we drop the superscript $j$ here for brevity):
$$\bm(s_i): \mathcal{S} \mapsto \mathcal{R}^{K}, \quad
\br(s_i): \mathcal{S} \mapsto \mathbb{P}(\GG_\alpha).$$ \lpk{what's the $\mathbb{P}$ stands for here?} In other words, we
define $\mathbf{RNN}(\bm(s_i), \br(s_i))$ as a recurrent network that takes a
fixed embedding input and a {\em set} of recurrent inputs from the global state,
both determined via a pre-specified function of the discrete state $s_i$. Note
that $K$ here is the fixed dimensionality of the input embedding, but the size
of the set returned by $\br$ can be dynamically sized.
\lpk{The notation $\mathbf{RNN}(\bm(s_i), \br(s_i))$ here looks like we are using a dynamically sized vector $\br(s_i)$ to replace the original $\bh_{i-1}$ (the previous hidden state in a RNN cell). Is that what's really happening? Or do we pull arbitrary hidden states and then concatenate them with $\bm(s_i)$? The previous hidden state dimension is dynamically sized sounds a little weired to me...}
\end{itemize}

From this definition, we see that executing this neural program will result in
an {\em acyclic graph} of computation. The edges in the graph are determined by
$\br$, which in turn is a function of the decisions in the transition
systems. Thus, the graph structure is {\em dynamic} and may not be a
deterministic function of the input. Finally, each link represents a {\em
  recurrence} in a deep neural network. Thus, we call this framework {\em
  dynamic recurrent acyclic graphical neural networks} (DRAGNN). 

We then define a DRAGNN {\em component} as the following extension of a TBRU:
\begin{itemize}
\item A {\em transition system}, $\mathcal{T}$,
\item A {\em network cell}, $\mathbf{RNN}$,
\item A {\em input} embedding function, $\bm$,
\item A {\em recurrent link} generating function, $\br$.
\end{itemize}
A DRAGNN is then an ordered collection of DRAGNN components. Note that we can
design particular components to capture particular aspects of the input or
output. Furthermore, this framework is inherently multi-task at multiple levels
of granularity: each transition system can produce zero to any number \lpk{finite?} of outputs
(e.g. joint parsing + tagging.)

The key aspect of this approach is to incorporate differentiable and
non-differential aspects according to the goals of the architecture
designer. Given a DRAGNN execution graph, gradients can be computed with respect
to each component's parameters via back-propagation. However, the design of
$\bm$ and $\br$ is not differentiable: they are functions of the discrete state,
which breaks backpropagation \lpk{break backpropagation made it sounds like this is not trainable?
Is there better way of saying that?}. Nonetheless, we will see that mixing
differentiable and non-differentiable components is an extremely effective tool
in practice. 

Note that the structure of the network cell is left vague by design. For
example, if the network cell includes an attention mechanism, that attention
could be defined over the input embeddings $\bm$ or a variable number of
recurrent links $\br$ (i.e. from another component).

\subsubsection{Examples}

% We make a few observations about the
% transition-based approach above:
% \begin{itemize}
% \item 
% \item To handle structure in the output of a , we can 
% \end{itemize}

%  By updating
% the transition system in the decoder, we can model arbitrary internal
% structure. For example:
% \begin{itemize}
% \item For tagging problems, we know that each output label corresponds to one
%   input token. We can use a transition system that produces exactly one tag per
%   token.
% \item For parsing problems, we know the output must form a hierarchical tree
%   structure. We can use a SHIFT/REDUCE transition system.
% \end{itemize}

% TODO: [Say something about attention]. Justify why we want to also change $\bm$:
% \begin{itemize}
% \item Tagging: Set the input $\bm(s_i) = \bh^E_{b}$ to be the encoder's
%   representation of the next input token in the parser's buffer.
% \item Parsing: Set the input $\bm(s_i) = \bh^E_i$ to be the encoder's
%   representatation of token $i$.
% \end{itemize}

% TODO: From stackprop: decoders can also be encoders. So we really just have an arbitrary list of components.  Then: Make $m$ pull more than one representation: can pull from the current component.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:

